Modeling Deontic Modal Logic in ASP

We consider the problem of implementing deontic modal logic. We show how (deontic) modal operators can be elegantly and directly expressed using default negation (negation-as-failure) and strong negation present in answer set programming (ASP). We propose using global constraints of ASP to represent obligations, prohibitions, and permissions in deontic modal logic. We show that our proposed representation results in the various decades-old paradoxes of deontic modal logic being simply and elegantly resolved. Our method also serves as a means for modeling conditional obligations and conditional prohibitions in knowledge representation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{325}
\providecommand{\publicationstatus}{W. Faber, L. Giordano, R. Rocha, V. Santos Costa (Eds.):\\ 42nd International Conference on Logic Programming (ICLP 2026)\\
EPTCS 450, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.450.25}{10.4204/EPTCS.450.25}}
\pdfoutput=1

